AttentiveNAS: Improving Neural Architecture Search via Attentive Sampling

Neural architecture search (NAS) has shown great promise in designing state-of-the-art (SOTA) models that are both accurate and efficient. Recently, two-stage NAS, e.g. BigNAS, decouples the model training and searching process and achieves remarkable search efficiency and accuracy. Two-stage NAS requires sampling from the search space during training, which directly impacts the accuracy of the final searched models. While uniform sampling has been widely used for its simplicity, it is agnostic of the model performance Pareto front, which is the main focus in the search process, and thus, misses opportunities to further improve the model accuracy. In this work, we propose AttentiveNAS that focuses on improving the sampling strategy to achieve better performance Pareto. We also propose algorithms to efficiently and effectively identify the networks on the Pareto during training. Without extra re-training or post-processing, we can simultaneously obtain a large number of networks across a wide range of FLOPs. Our discovered model family, AttentiveNAS models, achieves top-1 accuracy from 77.3% to 80.7% on ImageNet, and outperforms SOTA models, including BigNAS and Once-for-All networks. We also achieve ImageNet accuracy of 80.1% with only 491 MFLOPs. Our training code and pretrained models are available at https://github.com/facebookresearch/AttentiveNAS.

==> tex/related.tex <==


\subsection{Pareto-Aware NAS}
Pareto optimality is a situation where no individual or preference criterion can be better off without making at least one individual or preference criterion worse off.
The Pareto frontier is the set of all Pareto efficient allocations, shown in Figure \ref{fig:pareto_set}.
% 
Finding the Pareto frontier is generally NP-hard \cite{qian2015subset, davis1997adaptive}, which is usually solved by greedy algorithms \cite{davis1997adaptive} and convex relaxation methods \cite{tibshirani1996regression}.

Pareto-aware NAS \cite{elsken2018efficient, dong2018dpp} finds the Pareto set of architectures for the multi-objective (e.g. accuracy, flops) optimization on a proxy task and then train the found architectures from scratch.
These approaches still suffer from the gap between proxy searching and final training.
Moreover, the black-box searching algorithms, e.g. evolutionary algorithm~\cite{elsken2018efficient}, Bayesian optimization~\cite{dong2018dpp} do not perform good enough for the high-dimension optimization.
Therefore, the found architectures do not have enough improvement over random sampling or other simple baselines \cite{ying2019bench}.

